Well-posedness and potential-based formulation for the propagation of hydro-acoustic waves and tsunamis

We study a linear model for the propagation of hydro-acoustic waves and tsunami in a stratified free-surface ocean. A formulation was previously obtained by linearizing the compressible Euler equations. The new formulation is obtained by studying the functional spaces and operators associated to the model. The mathematical study of this new formulation is easier and the discretization is also more efficient than for the previous formulation. We prove that both formulations are well posed and show that the solution to the first formulation can be obtained from the solution to the second. Finally, the formulations are discretized using a spectral element method, and we simulate tsunamis generation from submarine earthquakes and landslides.

==> todo.tex <==
1
- The  velocity  and  the  density  must  satisfy  some  positivity  properties 
 C'est bizarre car la vitesse doit pouvoir être négative non ?

- Here  the  stress is a pressure, and is proportional to the divergence of the velocity field
je ne vois pas quelle équation montre ca?


3.1 
-The natural idea for writing the variational formulation associated to \eqref{eq:P:PDE_Vol}-\eqref{eq:P:PDE_Vol2} 
consists in testing \eqref{eq:P:PDE_Vol}-\eqref{eq:P:PDE_Vol2} against a function 
pourquoi les appeler comme $\varphi, \psi$, c'est parce que c'est les duals ?



6.2.2
- le point important est que les effets (rotationels si je ne me  trompe pas) qui ne sont pas présents dans la formulation potentiel sont vraiment négligeables. 
Peux-tu tester avec un déplacement beaucoup plus important : 5 m avec une vitesse beaucoup plus élevée et avec une partie qui monte à gauche par exemple et une partie qui descend à droite ? 
Peut-être que les effets rotationels seront plus importants ? 
Au moins on pourra comparer.

- les vitesses de soulèvements réelles semblent beaucoup plus rapides : https://agupubs.onlinelibrary.wiley.com/doi/full/10.1029/2019JB018946, il serait bien de tester quelque chose de plus réaliste ? 
Dans ce papier ils donnent des scénarios de glissement.

- il serait bien de superposer nos simulations avec potentiel aux siennes pour être plus quantitatif sur la comparaison

- ca me semble bizarre, je n'attendais pas de déformation de la surface libre aussi grande en lien avec les ondes acoustiques mais je me trompe visiblement...



6.3
- pourrait-on représenter la source pour que ce soit plus concret ? 
Quel est le déplacement max et sa vitesse ? 
Est-ce que les termes rotationels pourraient avoir une influence sur les ondes acoustiques ?



6.4
- Tu vas jsuqu'à zéro ? 
Tu pourrais prendre une amplitude de l'ordre de grandeur des signaux montrés dans les articles de Caplan en prenant le sismomètre le plus proche et en retrouvant un ordre de grandeur de l'amplitude à la source en supposant que l'atténuation de l'amplitude est en 1/r, on pourra dire que de toute facon l'équation des ondes est linéaire c'est juste pour avoir des valeurs à peu près réalistes

- peux-tu représenter le $\Delta f$ sur la figure 14 ?

- j'aurais aussi montré la vague de tsunami pour illustrer qu'on simule les deux à la fois.


%\begin{cases}
%- \dfrac{2 s_x r_x x}{(x-x_0)^2-r_x^2} %\exp \left(s_x  + \dfrac{s_x %r_x}{(x-x_0)^2 - r_x^2} \right), 
%& |x-x_0| \leq r_x
%\\
%0, &|x-x_0| > r_x
%\end{cases}, 
